Fast and Accurate Graph Stream Summarization

A graph stream is a continuous sequence of data items, in which each item indicates an edge, including its two endpoints and edge weight. It forms a dynamic graph that changes with every item in the stream. Graph streams play important roles in cyber security, social networks, cloud troubleshooting systems and other fields. Due to the vast volume and high update speed of graph streams, traditional data structures for graph storage such as the adjacency matrix and the adjacency list are no longer sufficient. However, prior art of graph stream summarization, like CM sketches, gSketches, TCM and gMatrix, either supports limited kinds of queries or suffers from poor accuracy of query results. In this paper, we propose a novel Graph Stream Sketch (GSS for short) to summarize the graph streams, which has the linear space cost (O(|E|), E is the edge set of the graph) and the constant update time complexity (O(1)) and supports all kinds of queries over graph streams with the controllable errors. Both theoretical analysis and experiment results confirm the superiority of our solution with regard to the time/space complexity and query results' precision compared with the state-of-the-art.

==> algorithm.tex <==
\section{Algorithm}
\label{sec:algorithm}
\subsection{Problem definition}
%In order to store the frequencies of items from \emph k sets, the naive method is to use \emph k CM sketches, one for each set. But there are drawbacks in this method. On most occasions, the requirement is to determine which set an item belongs to or find the set an item appears the most times, etc. In other words, we need to get the frequencies of an item in all the sets in a single query. Using the method described above, if there are \emph k sets and \emph d sub-tables in each CM sketch, \emph {d*k} hash functions and \emph {d*k} memory accesses will be needed, which can be considerably time consuming. In order to improve the performance of the system under these circumstances, we propose a new scheme based on CM sketch, which can reduce the number of hash functions and memory accesses needed, while keeping the accuracy unchanged. The algorithm and some mathematic analyses will be shown in this section.

%In the following part of the article, we assume that there are \emph k sets, ${{s}_{1}},{{s}_{2}}......{{s}_{k}}$.  the number of items in the ${i_{th}}$ set is ${{n}_{i}}$ and \emph N is the number of items in ${S={s}_{1}\cup {s}_{2}\cup {s}_{3}\cup ......\cup {s}_{k}}$. And we use ${r_{il}}$ to represent the value we get when querying the scheme for the frequency of the ${i_{th}}$ item in the ${l_{th}}$ set, and ${a_{il}}$ to represent the accurate frequency. As showed above, for single set, when the width of the CM sketch is$\lceil \frac{e}{\epsilon }\rceil$, and the number of sub-tables is $\lceil ln\frac{1}{\delta }\rceil$, then there will be a guarantee that ${Pr({r}_{i}\leq {a}_{i}+\epsilon ||s||)\geq 1-\delta }$ ,where  ${r_{i}}$  is the value we get when querying the scheme for the frequency of the ${i_{th}}$ item , ${a_{i}}$  is the accurate frequency and ${||s||=\sum_{i=1}^{n}{a}_{i}}$.Thus if all the ${{s}_{l}}$ ${1\leq l\leq k}$ share the same requirement on error${{r}_{i}-{a}_{i}}$,  and depth of CM sketches \emph d, the width of CM sketch needs to be linear correlative with ${||s||}$, which means the number of elements in the set.We assume the width of the ${l_{th}}$ CM sketch needs to be at least ${w_{l}}$, depending on ${||s_{l}||}$. And the depth of each CM sketch, in other words, number of sub-tables, is always \emph d.

Before describing our data structure in detail, we will first give a definition of the problem we attempt to solve. As stated above, a graph stream is a sequence of data with the form of $(s, d, w)$ where $s$ and $d$ are the IDs of the source node and the destination node, and $w$ is the set of attributes. $w$ may be composed of several attributes or none. An edge $(s, d)$ may appear in the sequence multiple times with different attribute sets. The attribute sets of the same edge can be cumulated with a predefined function. In this paper we assume that $w$ contains one attribute, and the function to cumulate the attributes is addition. When there are multiple attributes, we just deal with them separately.
%The stream graphs can be directed or undirected. In the following parts we focus on the directed graph, because the undirected graph can be seen as a special case of the directed graph where each edge in the undirected graph represents two edges with the same vertices and reversed directions There are many queries can be done.
In this paper we consider $3$ basic queries as examples:

1) Edge queries. An edge query means given an edge $(s, d)$, we want to get its attribute $w$. If the edge is not inserted in the data structure, we report $0$ instead. This is the most basic query in a graph.
%In practice an edge query may aim to find out the interaction frequency between two users or get the number of packets between two hosts. Some superior queries are combinations of several edge queries, like finding the minimum attributes in a path or a subgraph. As it is easy to handle them when edge queries are supported, we do not discuss them in this paper.

2) Node queries. An node query means given a node $s$, we want to find out the summary of the attributes of all edges emitted by this node. The node query is also an import query in applications which can help to evaluate the behavior of a node.
%For example, in a network traffic graph where the attribute of an edge represents the number of packets, the query result of an node is the total number of packets it sends and can be used to determine whether this host is a spiteful attacker.

3) Reachability queries. A Reachability query means given a pair of node $s$ and $d$, we need to check if there is a path from the source node to the destination node. It is the basic unit for many more complicated queries and also holds its place in applications.
%For example, finding out if the information sent from one host can reach another demands a reachability query.

\subsection{Basic Version}

The first novel technique of \fname\ is to introduce fingerprints into the summarization.
We build a matrix with the size of $m \times m$, and in \fname\ a node $s$ will get a hash value $h(s), (0 \leqslant h(s) \leqslant w-1)$ and a fingerprint $f(s)$. An inserted edge $(s, d)$ will be stored in the bucket in row $h(s)$, column $h(d)$ just like in TCM, but it will also be marked with a pair of fingerprints $f(s)$ and $f(d)$. Therefore each bucket in the matrix is composed of two fingerprints and a set of attributes. There are hash address collisions in the matrix, which means different edges are mapped into the same bucket. To store them, we enlarge each bucket into several rooms, each room can contain an edge. The inserted edge will occupy the leftmost empty room in the bucket it is mapped to. If there are no empty ones, it will be stored in a buffer which is composed of adjacency lists. In the adjacency lists we do not store the original IDs which can be very large. Instead we use $h(s)$ and $f(s)$ to represent a node $s$. The new key for $s$ is computed as $k(s) = h(s) \times F + f(s)$, where $F$ is the maximum value of the fingerprints.

When querying the \fname, we can check the fingerprint pair in each room to find out if it contains the edge we need.
In edge query for edge $(s, d)$, we first compute$h(s)$ and $h(d)$, and find the bucket in row $h(s)$, column $h(d)$. Then we check the rooms in this bucket. If we find an room with fingerprint pair $(f(s), f(d))$, we report the attributes stored in it. Otherwise we report that we do not find the edge.
In node query for node $v$, we can search the row it is mapped, and add up the attributes in the rooms where the first fingerprint in the pair is $f(v)$.
Similarly, in a breadth first search algorithm for reachability query from $s$ to $d$, when we need to find the nodes

It will avoid a lot of errors. For example, in edge query for $(s, d)$, if there is no such an edge in the graph, but there is an edge $(t, d)$, and $h(t)=h(s)$, then in TCM the query result will be attributes of edge $(t, d)$, while in \fname, this error can be avoided unless $f(s)=f(d)$. Similarly, in reachability query from $s$ to $d$, if $s$ can not reach $d$, but $t$ can reach it, and $h(s)=h(t)$, the answer of TCM will be wrong. The probability that there is at least one node $t$ satisfies $h(s)=h(t)$ and $t$ can reach $d$ is high, because there may be millions of nodes in the graph, while the value range of $h(.)$ is only thousands. Even if there is no such $t$, if a node $t'$ satisfies $h(t')=h(a)$, where $a$ is a node $s$ can reach, and $t'$ can reach $d$, the answer will still be wrong. Therefore in TCM the accuracy of reachability queries is not optimistic. While in \fname, node $s$ and $t$ will be mixed up only if $h(s)=h(t)$ and $f(s)=f(t)$, otherwise we will find out when checking the fingerprint pairs. As the fingerprints are randomly generated and can be 12-bit or even 16-bit, the probability of this situation is very small.

%The number of rooms in each bucket is usually $3$ or $4$. In this version there will still be too many edges stored in the buffer.
%Furthermore, when the distributions of node degrees is skewed in the graph as stated above, the rows which the nodes with high degrees are mapped to will be very crowded. This will not only lead to a larger buffer, but also cause a decrement in accuracy. Because the edges with one common node have much higher probability to have the same fingerprint pair, and if these edges squeezed together, there will be a higher probability of mistaking. In order to address these problems, In the following versions we introduce \hashname\ technique, it will provides multiple independent addresses for each edge, and this edge can be stored in the first empty room in these addresses. It will also spread the edges of one node among several rows, which will ease the congestion.

The structure of the basic version of the matrix in \fname is as follows:

\begin{figure}[htb]
\centering
\includegraphics [width=\figwidtheva]{V1.pdf}
\prefigcaption
\caption{Structure of the basic version of \fname}
\label{fig:V1}
\end{figure}

\subsection{Modified Version}

There are two main shortcomings of the basic version of \fname:
1) There is always skewness in the node degrees of a graph in practice. If a node $s$ emits many edges, the row $h(s)$ will be very crowded. This will cause both inaccuracy and a large buffer.
2) The probability of insertion failure in the matrix is high. If too many edges are inserted into the buffer, the linked lists will become very long. When traversing these linked lists to find an edge, a lot of time will be consumed.


In order to improve its performance, we introduce the second technique called \hashname. In \hashname, we map each edge into several buckets in the matrix rather than just one bucket. In this way there is a better chance that it find an empty room. Furthermore, after this improvement, instead of squeezing in a single row, the edges emitted by the high degree node are dispersed into several rows, which will ease the congestion. To accomplish this, we replace the hash address $h(s)$ and $h(d)$ in the basic version into two hash address sequences $\left \{h_i(s)\right \}$ and $\left \{ h_i(d) \right \}$ with $r$ independent hash addresses in each sequence. In this way we can get $r^2$ locations for edge $(s, d)$ with the address of $\left\{(h_i(s), h_j(d))|1 \leqslant i \leqslant r, 1\leqslant j \leqslant r \right\}$. we call these buckets the mapped buckets for convenience. We traverse these buckets and store the edge in the first one with empty rooms.

The method to generate the hash address sequence is not easy to find. %Because some iterative queries demand us to recover the full hash address sequences of the two endpoints given the position and content of a room. For example, in a reachability query from $s$ to $d$, we find that there is no edge $(s, d)$, but we do find an edge emitted by $s$ in the matrix. Then we need to check if the destination node of this edge $v$ can reach $d$. This demands us to recover the hash address sequence of $v$ to find all the positions $(v, d)$ may be stored. It is impossible if the hash address sequence is generated by a set of independent hash functions with the node ID as input. Because all the information we can get from a room is one hash address and the fingerprint of the node, and we can not get the result of other hash functions. And if we use the fingerprint as the input to carry out several hash functions, we can recover the hash address sequence, but the node with the same fingerprint will always get the same sequence, which will increase the probability of hash collisions and decrease the accuracy. Our approaches to generate the hash address sequence for a node $s$ is as following:
We hope that the addresses in the sequence is independent with each other, but if the hash address sequence of each node is generated by several independent hash functions with the node ID as the input, some queries can not be supported. In some topology queries such as a reachability query from $s$ to $d$, we need to carry out a recursive query: if we can not find edge $(s, d)$, we need to check if the nodes connected to $s$ can reach $d$, and further check their connected nodes if necessary. In this procedure, we need to search the rows $s$ is mapped, and find all the edges $s$ emitted. However, when we find such an edge, all the information we known about the destination node of this edge is a column index, which is one of the hash addresses of the destination node, and a fingerprint of the destination node. We do not want to store the node ID as it is usually very large. With these information, we can not recover the full hash address sequence of this node, thus can not check if it has an edge to $d$. On the other hand, if the hash address sequence is generated with the fingerprint of the node, the node with the same fingerprint will always get the same sequence, which makes it easier to mix them up. Therefore, in \hashname, this sequence of node $v$ is generated with a mixture of an original hash address $h(v)$ and its fingerprint $f(v)$. The procedure is as following:
%It works for simple queries like edge queries and node queries, but there are issues need to be settled in more complicated queries like reachability queries. These queries are often iterative and demand us to recover the full hash address sequences of the two endpoints given the position and content of a room. For example, in a reachability query from $s$ to $d$, we find that there is no edge $(s, d)$, but we do find an edge emitted by $s$ in the matrix. Then we need to check if the destination node of this edge $v$ can reach $d$. This demands us to recover the hash address sequence of $v$ to find all the positions $(v, d)$ may be stored. It is impossible if the hash address sequence is generated by a set of independent hash functions with the node ID as input. Because all the information we can get from a room is one hash address and the fingerprint of the node, and we can not get the result of other hash functions. And if we use the fingerprint as the input to carry out several hash functions, we can recover the hash address sequence, but the node with the same fingerprint will always get the same sequence, which will increase the probability of hash collisions and decrease the accuracy. Our approaches to generate the hash address sequence for a node $s$ is as following:

First we compute an original hash address $h(v)$ and a fingerprint $f(v)$.

Then we use linear congruence method to generate a sequence of $r$ random values $\left \{q_i(v)|1 \leqslant i \leqslant r \right \}$ with $f(v)$ as seed. The linear congruence method is as following: select a timer $a$, small prime $b$ and a big prime $p$, then $q_i(v)=(a \times q_{i-1}(v)+b)\% p, 2 \leqslant i \leqslant r$, and $q_1(v) = (a\times f(v)+b)\%p$. By choosing $a$, $b$ and $p$ carefully, we can make sure the cycle of the sequence we generate is much larger than $r$, and there will be no repetitive numbers in the sequence.

At last we generate a sequence of hash addresses as following: $\left \{h_i(v)| h_i(v) = (h(v)+q_i(v))\%m, 1\leqslant i \leqslant r \right \}$.

In the room an edge $(s, d)$ find as stated above, besides storing the pair of fingerprints and the attribute, we also store an index pair $(c_1, c_2)$, suppose that the bucket that contains this room has an address $(h_{c_1}(s), h_{c_2}(d))$. As the length of the sequence, $r$, is small, the length of each index will be less than $4$ bits. Therefore storing such a pair will cost little. Given the position and the content of the room, we can first compute sequences ${q_i(s)}$ and ${q_i(s)}$ with the fingerprints and the global variants $a$, $b$ and $p$. Then as we have the indexes of row and column of the bucket and index pair $(c_1,c_2)$, we can recover the original hash addresses $h(s)$ and $h(d)$, and compute the whole hash address sequences. By setting $p$ bigger than $m$, we can make sure that we get a unique solution in the above process.

The structure of the modified matrix of \fname\ is shown as follows:

\begin{figure}[h]
\centering
\includegraphics [width=\figwidtheva]{V2.pdf}
\prefigcaption
\caption{Structure of the modified version of \fname}
\label{fig:V2}
\end{figure}

\subsection{Improve the Speed}

There are further improvements to reduce the hash computation and memory access cost of \fname. First, we need to generate two values for a vertex $s$, the hash address $h(s)$ and the fingerprint $f(s)$, but we do not have to compute two independent hash functions. The hash addresses are within the range of $[0, m)$, where $m$ is the side length of the matrix. The matrix we build is usually not large, with a side length of thousands and even hundreds. This means the hash addresses we need are no more than $16$ bits. The fingerprints we generate are also no larger than $16$ bits. Therefore we can compute only one hash function $H(s)$, and then set $f(s) = H(s) \%F $, $h(s) = (H(s)/F)\%w$, where $F$ is the maximum value of fingerprints. Second, if we check all the $r \times r$ buckets as stated above, it will be very time-consuming. We can just choose a few buckets among them. We can not choose these buckets randomly, because when an edge comes in the graph stream, we need to check if it has already been inserted into the matrix. The buckets that we choose for the same edge in different times must be the same. In \fname, we add the fingerprints of the two vertices of an edge to get a seed, and use linear congruence method to produce a sequence with $k$ numbers in the range of $[0, r_2-1]$. This sequence will indicate $k$ buckets among the $r \times r$ buckets. We only search these buckets to find empty rooms. We call these $k$ buckets the candidate buckets. Experiments show that when $r=8$ and $k=8$ it is enough for most data sets. Last but not least, as stated above, in a bucket there are several rooms, and each room contains an index pair, a fingerprint pair and an attribute. Instead of maintaining separated rooms, we store all the index pairs in this bucket together at the front, and then follows all the fingerprint pairs, and at last there are the attributes. These three parts have the same storage order, in other words, the $i_{th}$ index pair, the $i_{th}$ fingerprint pair and the $i_{th}$ attribute belong to the same edge. When we check this bucket to find certain edges or empty positions, we can first check all the index pairs. If we find a matched index pair, we check the corresponding fingerprint pair, and if the fingerprint pair is also matched, we fetch the corresponding attributes. If we do not find any matched index pair, we can just move on and do not need to check the fingerprint pairs any more. As the index pairs are very small, usually no more than $8$ bits, we can fetch all the index pairs in one memory access. This improvement will accelerate the update and query process a lot as it omits a lot of memory accesses. After these improvements, the update speed of \fname is over $2$ millions updates per second in our experiments.
The matrix of the final version is shown in the following graph:

\begin{figure}[h]
\centering
\includegraphics [width=\figwidtheva]{V3-new.pdf}
\prefigcaption
\caption{Structure of the final version of \fname}
\label{fig:V3}
\end{figure}


\subsection{Update and query algorithm}

In this part we give an illustration of the updating and query process of the final version of \fname.  We use $m$ to represent the side length of the matrix, and in each buckets of the matrix there are $l$ rooms. The maximum value of the fingerprints is $F$. The hash address sequence we generate for a vertex has the length of $r$, and we choose $k$ candidate buckets for an edge. In practice we usually fixed $r=8$, $k=8$ and $l=4$ for most data sets. In some less skewed ones we can set $r=4$ to accelerate it. $m$ and $F$ can be set according to the size of the data set.
\subsubsection{Update}

Consider that in the graph stream a new data item $(s, d, w)$ comes, and the update progress will be as follows:

First, we compute hash function $H(s)$ and $H(v)$, and then generate fingerprint pair $f(s) = H(s) \%F $, $f(d) = H(d)\%F$, original hash address pair $h(s) = (H(s)/F)\%m$, $h(d) = (H(d)/F)\%m$.

Second, we use linear congruence method to produce two sequences
\begin{equation}
\left\{
\begin{aligned}
q_i(s)&=(a \times q_{i-1}(s)+b)\% p, 2 \leqslant i \leqslant r\\
q_1(s) &= (a\times f(s)+b)\%p\\
\end{aligned}
\right.
\end{equation}

and
\begin{equation}
\left\{
\begin{aligned}
q_i(d)&=(a \times q_{i-1}(d)+b)\% p, 2 \leqslant i \leqslant r\\
q_1(d) &= (a\times f(d)+b)\%p\\
\end{aligned}
\right.
\end{equation}

$a$, $b$ and $p$ are parameters of the linear congruence equation.

Third, we generate two sequences of hash addresses as following: $\left \{ h_i(s)| h_i(s) = (h(s)+q_i(s))\%m, 1\leqslant i \leqslant r \right \}$, and $\left \{h_i(d)| h_i(d) = (h(d)+q_i(d))\%m, 1\leqslant i \leqslant r \right \}$.

Fourth, we generate a sequence for this edge as
\begin{equation}
\left\{
\begin{aligned}
 Q_i=(a \times Q_{i-1}+b)\% p, 2 \leqslant i \leqslant k \\
 Q_1 = (a\times (f(s)+f(d))+b)\%p\\
 \end{aligned}
 \right.
 \end{equation}
 Then we choose $k$ buckets with address sequence $\left\{ (h_{\left \lfloor \frac{Q_i}{r}\%r  \right \rfloor}(s), h_{(Q_i\%r)}(d))| 1 \leqslant i \leqslant k \right\}$.

At last we check the rooms in the $k$ buckets by the order of the above sequence. Once we find a room in bucket $(h_{c_1}(s), h_{c_2}(d))$ with fingerprint pair $(f(s),f(d))$ and index pair $(c_1,c_2)$, we add $v$ to the value in the room and end the process. Otherwise if we find an empty room in in bucket $(h_{c_1}(s), h_{c_2}(d))$, we insert fingerprint pair $(f(s),f(d))$, index pair $(c_1,c_2)$ and $v$ in this room and end the process. Because every time we update this edge we will find the same $k$ buckets in the same order, this edge must be stored in the first bucket with empty rooms in the sequence. Therefore if we meet an empty room when traversing the address sequence before finding the queried edge, it means this edge has not been inserted into the matrix yet. We can just insert this edge in the room and end the process.

If we do not find the edge nor any empty room, we produce two keys $key(s)=h(s)\times F+f(s)$,  $key(d)=h(d)\times F+f(d)$, and insert this edge into the buffer which is a traditional adjacency list. Instead of storing original node IDs, we use these keys to represent the nodes in the adjacency list.

\subsubsection{edge query}

To answer an edge query for edge $(s, d)$, we perform the same process as updating and find $k$ buckets. Then we check the rooms in these buckets. If we find a room in bucket $(h_{c_1}(s), h_{c_2}(d))$ with fingerprint pair $(f(s),f(d))$ and index pair $(c_1,c_2)$, we return the value in this room as the result. If this edge can not be find in these $k$ edges, we search for $(key(s), key(d))$ in the adjacency lists in the buffer, where $key(s)$ an $key(d)$ are produced the same as stated above. We return the value in the buffer if we find the edge, otherwise we return $0$.

\subsubsection{node query}

To answer a node query for node $s$, we initialize the result with 0 and produce fingerprint $f(s)$ and hash address sequence $\left \{h_i(s) | i \leqslant i \leqslant r \right \}$. Then we check all the $r$ rows indicated by the hash address sequence. If a room in the $h_{c_1}(s)$ row has index pair $(c_1, c_{any})$ and fingerprint pair $(f(s), f_{any})$ where $c_{any}$ and $f_{any}$ could be any integers, we add the value in the room to the result. At last we check if there are edges with source node $key(s)$ in the buffer, and add their values to the result.

\subsubsection{reachability query}

Reachability query is the most complicated but the same important query discussed in our paper. There have been many prior works trying to answer reachability queries efficiently. like \cite{}, \cite{} and \cite{}. They can all be applied  in \fname. Here we use the most basic algorithm for reachability queries, the breadth-first search algorithm as an example. For a reachability query from source node $s$ to destination $d$, the process of BFS algorithm in \fname are as following: ($a$, $b$ and $p$ are all constants)
%\begin{algorithm}
%\caption{BFS code for reachability query}
%\Require source node $s$, destination node $s$
%\Ensure query result "True" or "False"

%\Function{LinearCongruence}{seed, length}
%    \State $q[0] \gets (seed \times a + b) \%p$
%    \State $i \gets 1$
%    \While{$i<length$}
%    \State $q[i] \gets (q[i-1] \times a + b) \%p$
%    \EndWhile
%    \State \Return{${q[i]}$}
%\EndFunction

%\Function{RecoverAddress}{f(y),j,c}
%    \State ${q_i(s)\gets LinearCongruence(f(y), r)}$
%    \While{$c\leqslant q_j(s)$}
%    \State $c=c+w$
%    \EndWhile
%    \State $h(s)=c-q_j(s)$
 %   \State \Return{$h(s)$}
%\EndFunction

%\end{algorithm}

We use keys which is generated as $key(s)=h(s) \times F+f(s)$, $key(d)=h(d) \times F+f(d)$ as stated above to present nodes in the graph in this procedure. We maintain a queue $Q$ of keys to store the nodes we need to search, and a set $S$ to store the keys we have already searched. $S$ is initialized to be empty, and $Q$ has only $key(s)$ at the beginning. We perform the search recursively. In each cycle, we fetch the top value $key(v)$ in $Q$ and pop $key(v)$ out from $Q$. Then we check if $key(v)$ is in $S$. If it is in $S$, we do nothing to it and move on to the next cycle. If not, we insert it to $S$ and recover $h(v)$ and $f(v)$ as $h(v) = key(v)/F$, $f(v)= key(v)\% F$. Then we can perform an edge query for edge $(v, d)$ as we already have $h(x)$, $f(x)$ and destination ID $d$. If we get an answer above $0$, we return a positive report and end the process. Otherwise, we generate the hash address sequence $\left \{ h_i(v)|1\leqslant i \leqslant r\right \}$ as stated above. and check all the $r$ rows indicated by this sequence. If a room in row $h_{c_1}(v)$ and column $C$ has fingerprint pair $(f(v), f(v'))$ and index pair $(c_1,c_2)$, it means there is an edge from $v$ to node $v'$, and $v'$ is a node we need to search in the following procedure. We can not recover node ID $v'$ with the information in the room, but we can compute $key(v')$. We use $f(v')$ to produce the sequence $\left\{q_i(v')\right\}$ as stated in the update section, and as $C=(h(v')+q_{c_2}(v'))\%m$ and $C \leqslant m, h(v') \leqslant m$, we can recover $h(v')$ with $q_{c_2}(v')$ and $C$. Then we generate $key(v')$ as $key(v')=h(v')\times F+f(v')$ and check if $key(v')$ is in $S$. If not we insert $key(v')$ to the end of $Q$, We should also check the buffer for any node linked to $key(v)$ and insert them to the end of $Q$ if they are not in $S$. We repeat this cycle until $Q$ is empty and return a negative report if we still do not find a node connected to $d$. This process is similar to the BFS algorithm in an adjacency matrix.
%We use one CM sketch to store the frequencies from all the sets, with a width of ${max({w}_{l})}$ ${1\leq l\leq k}$, and depth is d. But different from classic CM Sketch, we separate every basket in the Sketch into \emph k rooms, and there is a counter in each room. The counter in the ${{l}_{th}}$ room aims to store the frequency of the corresponding element in the ${{l}_{th}}$ set.

%When updating item \emph x in the ${{l}_{th}}$ set with increment \emph c($c=1$ when inserting, and -1 when deleting), set
%$\forall j \ 1\leq j\leq d \ count[j,{h}_{j}(x),l]=count[j,{h}_{j}(x),l]+c\ (1\leq l\leq k)$ ,where $count[j,{h}_{j}(x),l]$means the counter in the ${{l}_{th}}$ room of the basket ${{h}_{j}(x)}$ in the ${{j}_{th}}$ sub-table.

%In query of element \emph x, for the frequency in the ${{l}_{th}}$ set, we carry out hash functions and get$\forall j \ 1\leq j\leq d \ count[j,{h}_{j}(x),l]$ ,and return the minimum value as the result.

%The following graphic shows the data structure of the scheme:

%\includegraphics[width=3.00in,height=1.20in]{GraphVisio/version1.pdf}

%In this version of scheme, the number of hash functions and memory accesses have been reduced. Only \emph d hash functions are needed. And as the rooms in a basket are adjacent, and each counter is usually no more than 1 byte, we can get all the counters for an item in 1 or 2 memory accesses for each sub-table. This will optimize the speed of query when frequencies of an element from multiple sets are needed.

%But there are shortcomings in this version. The size of all the sets is not necessarily similar, and there even can be significant differences under some circumstances. This will lead to out-of-balance of the load factors in different rooms. Consider the situation that ${{n}_{i}\gg{n}_{j} }$,  as the accuracy for ${{s}_{i}}$  need to be guaranteed, the width of the sketch need to be larger than ${{w}_{i}}$ , which is much larger than ${{w}_{j}}$. This leads to a lot of 0 in the ${{j}_{th}}$ rooms,which is a waste of space.
%subsection{Time and Space Complexity}

%In this section we give a brief analysis about the time and space complexity about GCC.
\subsection {Mathematic Analyses}

In this section, we give a mathematical analysis about the correct rate of \fname when querying an edge and compare it to the correct rate of querying edges in TCM. As edge query is the basic unit of all the queries in graphs, this analysis will give a proof of the accuracy of \fname. We will also give an analysis of the possibility of the insertion failure of an edge in the matrix to show that the buffer area is usually very small.


There are two kinds of hash collisions in the \fname. The first kind is called the hash address collision, which means that two edges are mapped to the same bucket in the matrix, but with different fingerprint pairs or index pairs. In this case we will not mix these edges up and get wrong query answers, but if an edge has hash address collisions with other edges in all the candidate buckets, it will have no place in the matrix and have to be stored in the buffer. The second kind is called complete hash collisions, which means two different edges in the graph share at least one candidate bucket, and in this bucket they store the same fingerprint pair and index pair. In this case we can not separate these edges apart and may get wrong answers in query. The analysis of correct rate is to analyze the probability that two edges have complete hash collisions. We first prove the following theorem:
\begin{thm}\label{thm:1}
If two edges have complete hash collision in \fname, these two edges must have the same original hash address pair $(h(s), h(d))$ and the same fingerprint pair $(f(s), f(d))$.
\end{thm}
If two edges $e_1=(s_1, d_1)$ and $e_2=(s_2, d_2)$ share one candidate bucket in row $R$ and column $C$ in the matrix and have complete hash collision, they must have the same fingerprint pair, otherwise it will be easy for us to differentiate them. With the same fingerprints, these two edges will produce the same random value sequence ${q(s)}$ and $q(d)$. Moreover, this bucket must have the same index pair in the hash address sequences of these two edges, and we represent this pair with $(c_1, c_2)$. Then we have
\begin{equation}
\left\{
\begin{aligned}
 &(h(s_1)+q_{c_1}(s_1))\%m=R\\
 &((h(s_2)+q_{c_1}(s_2)))\%m=R \\
 &q_{c_1}(s_1)=q_{c_1}(s_2)\\
 \end{aligned}
 \right.
 \end{equation}
and
\begin{equation}
\left\{
\begin{aligned}
 &(h(d_1)+q_{c_2}(d_1))\%m=C\\
 &((h(d_2)+q_{c_2}(d_2)))\%m=C \\
 &q_{c_2}(d_1)=q_{c_2}(d_2)\\
 \end{aligned}
 \right.
 \end{equation}
With these equations, it is obvious that $h(d_1)=h(d_2)$, $h(s_1)=h(s_2)$ when $ 0 \leqslant h(s_1), h(s_2), h(d_1), h(d_2)< m$. With the same fingerprint pair and original hash addresses, these edges have no difference to us in \fname. We will store them in the same room and the query results we get for them will be the sum of their values.

Then we will calculate the correct rate when querying and edge $e$. We assume that there are $N_1$ edges in the graph which have no shared vertices with $e$, and $N_2$ edges with one shared vertex with $e$. In the following parts we call the first kind the non-adjacent edges of $e$, and the second kind adjacent edges of $e$ for convenience. We represent the side length of the matrix with $m$ and the maximum value of fingerprint with $F$. All the original hash addresses and fingerprints are generated randomly. For a non-adjacent edge of $e$, the probability that it has a complete hash collision with $e$ is the probability that this edge has the same original hash address pair and fingerprint pair as $e$, which is:
\begin{equation}
p_1 = \frac{1}{m^2 \times F^2}
\end{equation}
The probability that all the $N_1$ edges have no complete hash collisions with $e$ is
\begin{equation}
Pr_1={(1-p_1)}^{N_1}
\end{equation}
For those adjacent edges of $e$, as the original hash address and fingerprint of one node is already the same, the probability that such an edge has a complete collision with $e$ is
\begin{equation}
p_2 = \frac{1}{m \times F}
\end{equation}
The probability that all the $N_2$ edges have no complete hash collisions with $e$ is
\begin{equation}
Pr_2={(1-p_2)}^{N_2}
\end{equation}
Therefore the correct rate of $e$, in other words, all the $N_1+N_2$ edges do not have complete hash collisions with $e$ is
\begin{equation}
\begin{aligned}
Pr&=Pr_1 \times Pr_2\\
&=({(1-p_1)}^{N_1})\times ({(1-p_2)}^{N_2})\\
&=e^{-p_1 \times N_1} \times e^{-p_2 \times N_2}\\
&=e^{-\frac{N_1}{m^2 \times F^2}} \times e^{-\frac{N_2}{m \times F}}\\
&=e^{-\frac{N_1+m\times F\times N_2}{m^2 \times F^2}}\\
\end{aligned}
\end{equation}

When the size of the matrix has a linear correlation with the number of edges, this correct rate is very high. For example, suppose that the fingerprints we use are $16$-bit, in other words, $F=2^{16}$, and when querying an edge $e$, we have $N_1=1 \times 10^6$,$N_2=2000$. We use a matrix with side length $m=1000$. Then the correct rate of this edge query is $e^{-0.0000305}=0.99997$. In this case the graph is very highly skewed, as in real graph streams, the average degree of each node is usually smaller than $10$, which means the average number of adjacent edges of each node is less than $20$. Therefore in most queries the correct rate is much higher.

In TCM, if we also represent the side length of the matrix with $m$, and assume that there are $N_1$ edges with no common vertex with $e$ and $N_2$ edges share one vertex with $e$ in the graph, the correct rate of the query for $e$ in one matrix will be
\begin{equation}
\begin{aligned}
p'&={(1-\frac{1}{m^2})}^{N_1}\times {(1-\frac{1}{m})}^{N_2}\\
&={e}^{-\frac{N_1}{m^2}}\times {e}^{-\frac{N_2}{m}}\\
&={e}^{- \frac{N_1+m \times N_2}{m^2}}\\
\end{aligned}
\end{equation}
When $d$ independent matrices are used, the correct rate of TCM will be a combination of $d$ independent probability:
\begin{equation}
\begin{aligned}
Pr'&=1-{(1-p')}^d\\
&=1-{(1-{e}^{- \frac{N_1+m \times N_2}{m^2}})}^d
\end{aligned}
\end{equation}
When dealing the same edge query supposed as above,we set the side length of each matrix in TCM to $2000$, as the bucket in \fname\ is $10\sim 20$ times larger than TCM, and we allow TCM to use 4 matrices. In this case the total memory of TCM is already $3 \sim 4$ times larger than \fname. In such situation the correct rate of TCM is $0.741$ much lower than that of \fname. This gap will enlarge a lot in node queries and reachability queries, as they are aggregated by many edge queries. The performance will be further evaluated in the experiment part.

Then we consider the probability of insertion failure in the matrix. For the insertion of an edge $e$, we still suppose that there are already $N_1$ non-adjacent edges and $N_2$ adjacent edges inserted into the matrix. The side length of the matrix is $m$, and in each room there are $l$ rooms in each bucket. The length of the hash address sequence for each node is $r$, and for each edge we select $k$ candidate buckets. For each candidate bucket of $e$, as the non-adjacent edges are randomly mapped into the matrix with area $m^2$, the probability that there are $a_1$ non-adjacent edges mapped into it is:
\begin{equation}
\begin{aligned}
p_1(a_1)&=\binom{N_1}{a_1}\times {(\frac{1}{m^2})}^{a_1} \times {(1-\frac{1}{m^2})}^{N_1-a_1}\\
&=\binom{N_1}{a_1}\times {(\frac{1}{m^2})}^{a_1} \times {e}^{-\frac{N_1-a_1}{m^2}}
\end{aligned}
\end{equation}
As the adjacent edges are randomly mapped in an area of $r \times m$ ($r$ rows or $r$ columns in the matrix), the probability that there are $a_2$ adjacent edges mapped into this bucket is:
\begin{equation}
\begin{aligned}
p_2(a_2)&=\binom{N_2}{a_2}\times {(\frac{1}{r \times m})}^{a_2} \times {(1-\frac{1}{r\times m})}^{N_2-a_2}\\
&=\binom{N_2}{a_2}\times {(\frac{1}{r \times m})}^{a_2} \times {e}^{-\frac{N_2-a_2}{r\times m}}
\end{aligned}
\end{equation}
The probability that there are already $n$ edges inserted into this bucket is:
\begin{equation}
\begin{aligned}
p(n)&=\sum_{a=0}^{n}p_1(a)\times p_2(n-a)\\
\end{aligned}
\end{equation}
The probability that there are less than $l$ edges inserted into this bucket is:
\begin{equation}
\begin{aligned}
P&=\sum_{n=0}^{l-1}p(n)\\
&=\sum_{n=0}^{l-1}\sum_{a=0}^{n}p_1(a)\times p_2(n-a)\\
&=\sum_{n=0}^{l-1}\sum_{a=0}^{n}\binom{N_1}{a}\binom{N_2}{n-a}{(\frac{1}{m^2})}^{a}{(\frac{1}{rm})}^{n-a}{e}^{-\frac{N_1-a}{m^2}}{e}^{-\frac{N_2-n+a}{rm}}\\
\end{aligned}
\end{equation}
This is also the lower bound that the bucket is still available for $e$. The true probability is a little higher because when there are more than $l$ edges inserted into this bucket, they may occupy less than $l$ rooms because of fingerprint collision. But this probability is much smaller compared to the items in the formula above because the value range of fingerprints is large. Therefor we omit it in the formula. Then the probability that $e$ can not be inserted into the matrix is the probability that all the $k$ candidate buckets are not available, which is:
 \begin{equation}
\begin{aligned}
Pr=(1-P)^k
\end{aligned}
\end{equation}
Notice that this is an upper bound as we ignore fingerprint collisions here. This probability is rather small when the matrix is not too crowded. For example if $N_1=1\times 10^6$, $N_2=10^4$, we still set the side length of the matrix to $m=1000$, and set $r=8$, $l=3$, $k=8$, the upper bound probability of insertion failure is only $0.0022$. Experiments show that when the size of matrix is nearly equal to the number of edges, there will be almost no edges insert into the buffer. The details of the experiments will be shown in the next section.


==> experimentalresults.tex <==
\newcommand{\dataseta}{email-EuAll}
\newcommand{\datasetb}{web-NotreDame}
\newcommand{\datasetc}{cit-HepPh}
\section{Experimental Results}
\label{sec:experimentalresults}
In this section, we show our experimental studies of \fname. We first explain the data sets in experiments (\ref{dataset}) and evaluation metrics (\ref{metrics}). Next, we compare \fname\ with TCM on three fundamental queries: edge query (\ref{edgequery}), node query (\ref{nodequery}) and reachability query (\ref{reachabilityquery}). We also evaluate the load factor of \fname\ (\ref{loadfactor}). Finally, we summarize our experimental studies (\ref{summary}).

All experiments are performed on a server with dual 6-core CPUs (Intel Xeon CPU E5-2620 @2.0 GHz, 24 threads) and 62 GB DRAM memory, running Ubuntu. All algorithms including \fname\ and TCM are implemented in C++.
\subsection{Data Sets}\label{dataset}
We choose three real data sets from Stanford Network Analysis Platform (SNAP)\footnote{http://snap.stanford.edu/data}. Details of three data sets are described as follows:

1)\textbf{\dataseta}\footnote{http://snap.stanford.edu/data/email-EuAll.html}.This data set is communication network data generated using email data from a large European research institution for a period of 18 months. Each node in the directed graph corresponds to an email address. Each edge between node \emph{src} and \emph{dst} represents \emph{src} sent at least one email to \emph{dst}. The directed graph contains 265214 nodes and 420045 edges. We use the Zipfian distribution to add the weight to each edge and the edge weight represents the appearance times in the stream.

2)\textbf{\datasetb}\label{dataset2}\footnote{http://snap.stanford.edu/data/web-NotreDame.html}.The second real data set is a web graph collected from the University of Notre Dame. Nodes represent web pages and directed edges represent hyperlinks between pages. The directed graph contains 325729 nodes and 1497134 edges. The edge weights are added using Zipfian distribution.

3)\textbf{\datasetc}\label{dataset3}\footnote{http://snap.stanford.edu/data/email-EuAll.html}.It is the Arxiv HEP-PH (high energy physics phenomenology) citation graph. If a paper \emph{src} cites paper \emph{dst}, the data set contains a directed edge from  \emph{src} to \emph{dst}. The data set covers  34,546 papers as nodes with 421,578 edges. The edge weights are also added using Zipfian distribution.

The function we use to cumulate the edge weights is addition. In such case, TCM and \fname\ only have over-estimations.

\subsection{Metrics}\label{metrics}
\textbf{Average Relative Error (ARE):} ARE measures the accuracy of the estimated attributes for the set of queries, such as edge or node queries. Given a query $q$, the \emph{relative error} is defined as
\[
\begin{aligned}
er(q) = \frac{\hat{f(q)}}{f(q)}-1
\end{aligned}
\]
where $f(q)$ and $\hat{f(q)}$ are the real attribute and the estimated attribute of $q$. When giving a query set $Q=\{q_1,q_2,...,q_k\}$, the \emph{average relative error} is measured by averaging the relative errors over all queries of $Q$:
\[
\begin{aligned}
ARE(Q) = \frac{\sum_{i=1}^ker(q_i)}{k}
\end{aligned}
\]
\textbf{Average Absolute Error (AAE):} In addition to the ARE, we also consider the AAE. Given a query $q$, the \emph{absolute error} is defined as
\[
\begin{aligned}
er(q) = \hat{f(q)}-f(q)
\end{aligned}
\]
where $f(q)$ is the real attribute of $q$ and $\hat{f(q)}$ is the estimated attribute of $q$. When giving a query set $Q=\{q_1,q_2,...,q_k\}$, the \emph{average absolute error} is measured by averaging the absolute errors over all queries of $Q$:
\[
\begin{aligned}
AAE(Q) = \frac{\sum_{i=1}^ker(q_i)}{k}
\end{aligned}
\]
\textbf{True Negative Recall:} It measures the accuracy of the reachability query. Because connectives of all edges are kept, there is no false positive in \fname. When giving a reachability query set $Q=\{q_1,q_2,...,q_k\}$,$\forall q_i\in Q$, node $src$ and node $dst$ in $q_i$ are unreachable. \emph{True negative recall} is defined as  the number of queries reported as unreachable divided by the number of all queries in $Q$.\\
%:
%\[
%\begin{aligned}
%r(Q) = \frac{t}{k}
%\end{aligned}
%\]
%Here, $t$ is the number of queries detected as unreachable over all queries of $Q$.
\textbf{Buffer Percentage:} It measures load factor of \fname. After all data items from the same graph stream are updated, we count the number of data items inserted in the buffer rather than the adjacency matrix. \emph{Buffer percentage} is defined as the number of items that the buffer contains divided by the total number of items in the same graph stream.
%\[
%\begin{aligned}
%r(Q) = \frac{t}{n}
%\end{aligned}
%%\]
\subsection{Experiments on edge query}\label{edgequery}
In this section, we evaluate the performance of \fname \ in estimating attributes of edge queries. We varied two parameters of \fname, \emph{fsize} that is the size of the fingerprint and \emph{width} that is the width of the matrix. Moreover, we compare \fname\  with TCM by fixing the ratio of the memory used by TCM and \fname\  8 times (i.e., TCM is 8 times the memory overhead of \fname). In all experiments , we implement TCM and \fname \  using square matrices. Because without a prior knowledge of graph stream distribution, it's difficult to decide a reasonable size of the non-square matrix.
\begin{figure}[htbp]
\subfigure[\dataseta]{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{EEedge-ARE.pdf}
\label{EEedge-ARE}
\end{minipage}
}
\subfigure[\datasetb]{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{WNedge-ARE.pdf}
\label{WNedge-ARE}
\end{minipage}
}
\subfigure[\datasetc]{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{citedge-ARE.pdf}
\label{citedge-ARE}
\end{minipage}
}
\caption{Average Relative Error of Edge Queries}\label{edgeARE}
\end{figure}

%\begin{figure*}
%\centering
%\includegraphics[width=0.32\textwidth]{EEedge-ARE.pdf}
%\includegraphics[width=0.32\textwidth]{WNedge-ARE.pdf}
%\includegraphics[width=0.32\textwidth]{citedge-ARE.pdf}
%\caption{Average Relative Error of Edge Queries}\label{edgeARE}
%\end{figure*}
%
%\begin{figure*}
%\centering
%\includegraphics[width=0.32\textwidth]{EEedge-AAE.pdf}
%\includegraphics[width=0.32\textwidth]{WNedge-AAE.pdf}
%\includegraphics[width=0.32\textwidth]{citedge-AAE.pdf}
%\caption{Average Absolute Error of Edge Queries}\label{edgeAAE}
%\end{figure*}

\begin{figure}[htbp]
\subfigure[\dataseta]
{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{EEedge-AAE.pdf}
\label{EEedge-AAE}
\end{minipage}
}
\subfigure[\datasetb]{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{WNedge-AAE.pdf}
\label{WNedge-AAE}
\end{minipage}
}
\subfigure[\datasetc]{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{citedge-AAE.pdf}
\label{citedge-AAE}
\end{minipage}
}
\caption{Average Absolute Error of Edge Queries}\label{edgeAAE}
\end{figure}

Fig. \ref{edgeARE} (Fig. \ref{edgeAAE}) show the ARE (AAE) of edge attributes estimation for the data sets \dataseta, \datasetb\  and \datasetc, respectively. For \fname, we fixed independent hash addresses in each sequences $r=8$, the number of candidate buckets $k=8$ and the number of rooms in each buckets $l=4$ for all three data sets. For TCM, the number of hash functions $d$ is fixed to be 4 for all three data sets. We tried to increase the number of hash functions, but TCM can not perform significantly better since with the same memory constraint we have to reduce the size of every matrix to achieve multiple hash functions. We varied the memory of \fname\  by different widths of the matrix. To be comparable with \fname, TCM is 8 times the memory overhead of \fname. If we fixed the sizes of TCM smaller, the performance of TCM in edge queries would be worse by too many orders of magnitude than \fname\  (e.g., when the memory overhead of TCM is the same as \fname, the ARE and the AAE of TCM in edge queries is higher by three or four orders of magnitude than \fname). To reduce random error introduced by the selection of the data sample, the edge query set Q contains all edges in the graph stream.

The above results tell us that \fname\  performs much better in supporting edge queries than TCM, even though TCM is 8 times the memory overhead of \fname. When fixing $fsize=16$ and $width=800$, the ratio that the ARE of \fname\ divided by the ARE of TCM is only  0.1\textperthousand\  and 2\textperthousand\ for the data sets \dataseta\ and \datasetb\ while the ARE of \fname\ is 0 in \datasetc. Moreover, since the scales of the data sets \dataseta \ and \datasetb \ are larger than the data set \datasetc, \fname \ outperforms TCM more significantly in figures \ref{EEedge-ARE} and \ref{WNedge-ARE} than in figure \ref{citedge-ARE}. It is because that \fname\ better spread the edges all over the matrix and introduce fingerprints to reduce collisions of different edges. So \fname\  can be better adapted to deal with the very large graph.

It is easy to understand the ARE and the AAE decrease along with the growth of the width of the matric. Also, when the length of fingerprint becomes longer, the AAE and ARE of \fname\  are lower. When the length of fingerprint is fixed to be 16 bits, the ARE and the AAE of \fname\  are almost 0 in all experiments on edge queries of three data sets.

\subsection{Experiments on Node Query}\label{nodequery}
In this section, we evaluate the performance of \fname \ in estimating the summary of the attributes of all edges emitted by one node. We varied two parameters of \fname, $fsize$ that is the size of the fingerprint and $width$ that is the width of the matrix. For \fname, we fixed independent hash addresses in each sequences $r=8$, the number of candidate buckets $k=8$ and the number of rooms in each buckets $l=4$ for all three data sets. For TCM, the number of hash functions $d$ is fixed to be 4 for all three data sets. Also, we fixed the ratio of the memory used by TCM and \fname \ 256 times (i.e.,
TCM is 256 times the memory overhead of \fname). Note that the ratio in the set of node query experiments is much higher than that, 8 times, in the set of edge query experiments. For each data set, node query set $Q$ contains all nodes in the graph stream.

\begin{figure}[htbp]
\subfigure[\dataseta]{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{EEnode-ARE.pdf}
\label{EEnode-ARE}
\end{minipage}
}
\subfigure[\datasetb]{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{WNnode-ARE.pdf}
\label{WNnode-ARE}
\end{minipage}
}
\subfigure[\datasetc]{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{citnode-ARE.pdf}
\label{citnode-ARE}
\end{minipage}
}
\caption{Average Relative Error of Node Queries}\label{nodeARE}
\end{figure}

%\begin{figure*}
%\centering
%\includegraphics[width=0.32\textwidth]{EEnode-ARE.pdf}
%\includegraphics[width=0.32\textwidth]{WNnode-ARE.pdf}
%\includegraphics[width=0.32\textwidth]{citnode-ARE.pdf}
%\caption{Average Relative Error of Node Queries}\label{nodeARE}
%\end{figure*}
%
%\begin{figure*}
%\centering
%\includegraphics[width=0.32\textwidth]{EEnode-ARE.pdf}
%\includegraphics[width=0.32\textwidth]{WNnode-ARE.pdf}
%\includegraphics[width=0.32\textwidth]{citnode-ARE.pdf}
%\caption{Average Relative Error of Node Queries}\label{nodeARE}
%\end{figure*}

\begin{figure}[htbp]
\subfigure[\dataseta]
{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{EEnode-AAE.pdf}
\label{EEnode-AAE}
\end{minipage}
}
\subfigure[\datasetb]{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{WNnode-AAE.pdf}
\label{WNnode-AAE}
\end{minipage}
}
\subfigure[\datasetc]{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{citnode-AAE.pdf}
\label{citnode-AAE}
\end{minipage}
}
\caption{Average Absolute Error of Node Queries}\label{nodeAAE}
\end{figure}

Fig. \ref{nodeARE} (Fig. \ref{nodeAAE}) show the ARE (AAE) of the estimated summary of the attributes of all edges emitted by each node in query set $Q$ for the data sets \dataseta, \datasetb \ and \datasetc, respectively. To make TCM comparable with \fname, we fixed the memory  of TCM 256 times as large as \fname. Although we unfairly fix the ratio of memory used by TCM and \fname, \fname\ still can achieve better performance than TCM.

The above results tell us that \fname\  consistently outperforms TCM in all data sets. When fixing $fsize=16$ and $width=800$, the ratio that the ARE of \fname\ divided by the ARE of TCM is only 5\textperthousand, 2\textperthousand\  and 2\textperthousand\  for the data sets \dataseta\ ,\datasetb\ and \datasetc, respectively. As Fig \ref{nodeAAE} and Fig \ref{nodeARE} show, \fname\ can outperform TCM more significantly in data sets with larger scale (\dataseta\ and \datasetb) than relatively smaller data set (\datasetc). With longer fingerprint length and larger memory, \fname\ can perform better. When $fsize$ is fixed as 16, the ARE and the AAE of \fname\  are almost 0 that are two or three orders of magnitude lower than those of TCM with 256 times more memory.

\subsection{Experiments on Reachability Query}\label{reachabilityquery}
In this section, we evaluate the performance of \fname\  in supporting reachability queries. We varied two parameters of \fname, $fsize$ that is the size of the fingerprint and $width$ that is the width of the matrix. For \fname, we fixed independent hash addresses in each sequences $r=8$, the number of candidate buckets $k=8$ and the number of rooms in each buckets $l=4$ for all three data sets. For TCM, the number of hash functions $d$ is fixed to be 4 for all three data sets. Also, we fixed the ratio of the memory used by TCM and \fname \ 256 times (i.e.,
TCM is 256 times the memory overhead of \fname). Since connectives of every edge in graph stream are stored in TCM and \fname, there is no false positive in TCM and \fname\ (i.e., any reachable pair of nodes will be reported as reachable). So reachability query set $Q$ only contains 100 unreachable pairs of nodes which are randomly generated from the graph. We use true negative recall that is the number of pairs of nodes reported as unreachable divided by 100 to measure the accuracy of the reachability query.
\begin{figure}[htbp]
\subfigure[\dataseta]{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{EEtrans.pdf}
\label{EEtrans}
\end{minipage}
}
\subfigure[\datasetb]{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{WNtrans.pdf}
\label{WNtrans}
\end{minipage}
}
\subfigure[\datasetc]{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{cittrans.pdf}
\label{cittrans}
\end{minipage}
}
\caption{True Negative Recall of Reachability Queries}\label{trans}
\end{figure}

%\begin{figure*}
%\centering
%\includegraphics[width=0.32\textwidth]{EEtrans.pdf}
%\includegraphics[width=0.32\textwidth]{WNtrans.pdf}
%\includegraphics[width=0.32\textwidth]{cittrans.pdf}
%\caption{True Negative Recall of Reachability Queries}\label{trans}
%\end{figure*}

Fig. \ref{trans} show the true negative recall of reachability query for the data sets \dataseta, \datasetb \ and \datasetc, respectively.
 When fixing $fsize=16$ and $width=800$, the true negative recall of \fname\  is 7.7, 11.6 and 2.7 times higher than TCM for the data sets \dataseta\ ,\datasetb\ and \datasetc, respectively. Even though TCM used 256 times the memory that \fname\ used, the accuracy of \fname\  for reachability queries is still much higher than TCM especially in relatively large data sets (\dataseta\  and \datasetb). Along with increasing the memory and the length of the fingerprint, \fname\  can achieve better performance. Fig.\ref{EEtrans} shows that when we fixed the length of fingerprint 16 bits, the true negative recall of \fname\ is consistently close to $100\%$.
\subsection{Experiments on Load Factor}\label{loadfactor}
In  this section, we evaluate the load factor of \fname. If an edge finds that all candidate buckets to are occupied, it will be stored in the buffer which is a traditional adjacency list. When all edges in a data set have been updated, we use the buffer percentage which is the number of edges in the buffer divided by the number of all edges to evaluate the load factor. For \fname, we fixed independent hash addresses in each sequences $r=8$, the number of candidate buckets $k=8$ and the number of rooms in each buckets $l=4$ for all three data sets. We varied the length of fingerprint and the width of the matrix.

\begin{figure}
\subfigure[\dataseta]{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{EEbuff.pdf}
\label{EEbuff}
\end{minipage}
}
\subfigure[\datasetb]{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{WNbuff.pdf}
\label{WNbuff}
\end{minipage}
}
\subfigure[\datasetc]{
\begin{minipage}[b]{0.5\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{citbuff.pdf}
\label{citbuff}
\end{minipage}
}
\caption{Buffer Percentage}\label{buff}
\end{figure}

%\begin{figure*}
%\centering
%\includegraphics[width=0.32\textwidth]{EEbuff.pdf}
%\includegraphics[width=0.32\textwidth]{WNbuff.pdf}
%\includegraphics[width=0.32\textwidth]{citbuff.pdf}
%\caption{Buffer Percentage}\label{buff}
%\end{figure*}

Fig. \ref{buff} show the buffer percentage for three data sets \dataseta, \datasetb \ and \datasetc, respectively. The above results tell us that the load factor of \fname\ is very high when the buffer percentage for three data sets is below $10^{-4}$. When fixing $fsize=16$ and $width=800$, the buffer percentage is only 0, $6.4\times10^{-5}$ and 0 for the data sets \dataseta\ ,\datasetb\ and \datasetc, respectively. If we fixed the width of the matrix relatively large, there is almost no item inserted in the buffer. For example, Fig.\ref{WNbuff} shows that only 4 items are in the buffer after 1497134 items from \datasetb\ are updated in \fname\ ($fsize=16,width=1000$). In this case, the overhead brought by the insertion failure in the matrix is nearly 0.

\subsection{Summary of Experimental Studies}\label{summary}
After extensive experiments of \fname\ and TCM on three data sets, we can make following conclusions:

1)\fname\ can perform much better than the state-of-the-art in supporting basic queries including edge query, node query and reachability query. In particular, \fname\ with less memory usage is still orders of magnitude better than TCM.

2)\fname\ is more resistent to the uneven distribution of node degrees by introducing fingerprint and mapping each edge into more than one buckets. So \fname\  can be a better solution to support most kinds of queries on very large graph streams.

3)The load factor of \fname\ is very high. So \fname\ has high memory efficiency.


==> implementation.tex <==
\section{implementation}
\label{sec:implementation}


